Marginal modeling of cluster-period means and intraclass correlations in stepped wedge designs with binary outcomes

Stepped wedge cluster randomized trials (SW-CRTs) with binary outcomes are increasingly used in prevention and implementation studies. Marginal models represent a flexible tool for analyzing SW-CRTs with population-averaged interpretations, but the joint estimation of the mean and intraclass correlation coefficients (ICCs) can be computationally intensive due to large cluster-period sizes. Motivated by the need for marginal inference in SW-CRTs, we propose a simple and efficient estimating equations approach to analyze cluster-period means. We show that the quasi-score for the marginal mean defined from individual-level observations can be reformulated as the quasi-score for the same marginal mean defined from the cluster-period means. An additional mapping of the individual-level ICCs into correlations for the cluster-period means further provides a rigorous justification for the cluster-period approach. The proposed approach addresses a long-recognized computational burden associated with estimating equations defined based on individual-level observations, and enables fast point and interval estimation of the intervention effect and correlations. We further propose matrix-adjusted estimating equations to improve the finite-sample inference for ICCs. By providing a valid approach to estimate ICCs within the class of generalized linear models for correlated binary outcomes, this article operationalizes key recommendations from the CONSORT extension to SW-CRTs, including the reporting of ICCs.

==> refs.tex <==
%DCSWD Citation
@preamble{ " \newcommand{\noop}[1]{} " } % a do-nothing command that serves a purpose

% B
@article{Baio2015,
author = {Baio, Gianluca and Copas, Andrew and Ambler, Gareth and Hargreaves, James and Beard, Emma and Omar, Rumana Z},
issn = {1745-6215},
journal = {Trials},
pages = {354-368},
pmid = {26282553},
publisher = {Trials},
title = {{Sample size calculation for a stepped wedge trial.}},
volume = {16},
year = {2015}
}

% C
@article{copas2015designing,
  title={Designing a stepped wedge trial: three main designs, carry-over effects and randomisation approaches},
  author={Copas, Andrew J and Lewis, James J and Thompson, Jennifer A and Davey, Calum and Baio, Gianluca and Hargreaves, James R},
  journal={Trials},
  volume={16},
  pages={352},
  year={2015},
  publisher={Springer}
}

% D
@book{Donner2000,
author = {Donner, Allan. and Klar, Neil},
howpublished = {Hardcover},
publisher = {Oxford University Press},
address={New York, NY},
title = {{Design and Analysis of Group-Randomized Trials in Health Research}},
year = {2000}
}

% E
@book{Eldridge2012,
author = {Eldridge, Sandra and Kerry, Sally},
howpublished = {Hardcover},
publisher = {John Wiley \& Sons},
address={Chichester, West Sussex},
title = {{A Practical Guide to Cluster Randomised Trials in Health Services Research}},
year = {2012}
}
@article{Eldridge2006,
author = {Eldridge, Sandra M. and Ashby, Deborah and Kerry, Sally},
journal = {International Journal of Epidemiology},
number = {5},
pages = {1292--1300},
title = {{Sample size for cluster randomized trials: Effect of coefficient of variation of cluster size and analysis method}},
volume = {35},
year = {2006}
}

% F
@article{Fay2001,
author = {Fay, M. P. and Graubard, B. I.},
journal = {Biometrics},
pages = {1198--1206},
title = {{Small-sample adjustments for Wald-type tests using sandwich estimators}},
volume = {57},
year = {2001}
}
@article{ford2020maintaining,
  title={Maintaining the validity of inference in small-sample stepped wedge cluster randomized trials with binary outcomes when using generalized estimating equations},
  author={Ford, Whitney P and Westgate, Philip M},
  journal={Statistics in Medicine},
  volume={39},
  pages={2779--2792},
  year={2020},
  publisher={Wiley Online Library}
}

% G
@article{Golden2015,
author = {Golden, M. R. and Kerani, R. P. and Stenger, M. and Hughes, J. P. and Aubin, M. and Malinski, C. and Holmes, K. K.},
journal = {Plos Medicine},
pages = {1--22},
title = {{Uptake and population-level impact of expedited partner therapy (EPT) on Chlamydia trachomatis and Neisseria gonorrhoeae: the Washington State community-level randomized trial of EPT}},
volume = {12},
year = {2015}
}
@article{Gannon-Loew2017,
author = {Gannon-Loew, K. E. and Holland-Hall, C. and Bonny, A. E.},
issn = {18734332},
journal = {Journal of Pediatric and Adolescent Gynecology},
pages = {341--348},
title = {{A review of expedited partner therapy for the management of sexually transmitted infections in adolescents}},
volume = {30},
year = {2017}
}

@article{Grantham2019,
author = {Grantham, K. L. and Kasza, J. and Heritier, S. and Hemming, K. and Forbes, A. B.},
journal = {Statistics in Medicine},
title = {{Accounting for a decaying correlation structure in cluster randomized trials with continuous recruitment}},
year = {2019},
pages = {1918--1934},
volume={38}
}

@article{Grayling2017b,
author = {Grayling, M. J. and Wason, J. M. S. and Mander, A. P.},
journal = {Trials},
pages = {1--13},
publisher = {Trials},
title = {{Stepped wedge cluster randomized controlled trial designs : a review of reporting quality and design features}},
volume = {18},
year = {2017}
}



% H
@article{Hin2009,
author = {Hin, L.-Y. and Wang, Y.-G.},
journal = {Statistics in Medicine},
pages = {642--658},
title = {{Working-correlation-structure identification in generalized estimating equations}},
volume = {28},
year = {2009}
}
@book{Hayes2009,
author = {Hayes, R. J. and Moulton, L. H.},
howpublished = {Hardcover},
publisher = {Taylor \& Francis Group, LLC},
address={Boca Raton, FL},
title = {{Cluster Randomised Trials}},
year = {2009}
}
@article{Hemming2015,
author = {Hemming, Karla and Lilford, Richard and Girling, Alan J.},
journal = {Statistics in Medicine},
pages = {181--196},
pmid = {25346484},
title = {{Stepped-wedge cluster randomised controlled trials: A generic framework including parallel and multiple-level designs}},
volume = {34},
year = {2015}
}
@article{Hemming2016,
author = {Hemming, Karla and Taljaard, Monica},
journal = {Journal of Clinical Epidemiology},
pages = {137--146},
publisher = {Elsevier},
title = {{Sample size calculations for stepped wedge and cluster randomised trials: a unified approach}},
volume = {69},
year = {2016}
}
@article{Hemming2018,
author = {Hemming, K. and Taljaard, M. and McKenzie, J. E. and Hooper, R. and Copas, A. and Thompson, J. A. and et al},
journal = {BMJ},
pages = {1--26},
title = {{Reporting of stepped wedge cluster randomised trials: Extension of the CONSORT 2010 statement with explanation and elaboration}},
volume = {363},
year = {2018}
}

@article{Hughes2015,
author = {Hughes, J. P. and Granston, T. S. and Heagerty, P. J.},
journal = {Contemporary Clinical Trials},
pages = {55--60},
publisher = {Elsevier Inc.},
title = {{Current issues in the design and analysis of stepped wedge trials}},
volume = {45},
year = {2015}
}
@article{Hussey2007,
author = {Hussey, M. A. and Hughes, J. P.},
journal = {Contemporary Clinical Trials},
pages = {182--191},
pmid = {16829207},
title = {{Design and analysis of stepped wedge cluster randomized trials}},
volume = {28},
year = {2007}
}
@article{Hooper2016,
author = {Hooper, Richard and Teerenstra, Steven and de Hoop, Esther and Eldridge, Sandra},
journal = {Statistics in Medicine},
pages = {4718--4728},
title = {{Sample size calculation for stepped wedge and other longitudinal cluster randomised trials}},
volume = {35},
year = {2016}
}
@article{Heagerty2000,
author = {Heagerty, P. J. and Zeger, S. L.},
journal = {Statistical Science},
pages = {1--19},
title = {{Marginalized multilevel models and likelihood inference}},
volume = {15},
year = {2000}
}
@article{Harrison2019,
author = {Harrison, Linda J. and Chen, Tom and Wang, Rui},
journal = {Biometrics},
title = {{Power calculation for cross-sectional stepped wedge cluster randomized trials with variable cluster sizes}},
pages = {Early View},
year = {2019}
}
@article{Heagerty1999,
author = {Heagerty, Patrick J},
journal = {Biometrics},
pages = {688--698},
title = {{Marginally specified logistic-normal models for longitudinal binary data.}},
volume = {55},
year = {1999}
}
@article{Heagerty2001,
author = {Heagerty, Patrick J. and Kurland, Brenda F.},
journal = {Biometrika},
pages = {973--985},
title = {{Misspecified maximum likelihood estimates and generalised linear mixed models}},
volume = {88},
year = {2001}
}
@article{hooper2019stepped,
  title={Stepped wedge trials with continuous recruitment require new ways of thinking},
  author={Hooper, Richard and Copas, Andrew},
  journal={Journal of Clinical Epidemiology},
  volume={116},
  pages={161--166},
  year={2019},
  publisher={Elsevier}
}

% S
@article{Simpson2010,
author = {Simpson, Sean L. and Edwards, Lloyd J. and Muller, Keith E. and Sen, Pranab K. and Styner, Martin A.},
journal = {Statistics in Medicine},
pages = {1825--1838},
title = {{A linear exponent AR(1) family of correlation structures}},
volume = {29},
year = {2010}
}
@article{Sharples1992,
author = {Sharples, K. and Breslow, N.},
journal = {Journal of Statistical Computation and Simulation},
pages = {1--20},
title = {{Regression analysis of correlated binary data: some small sample results for the estimating equation approach}},
volume = {42},
year = {1992}
}


% K
@article{Kauermann2001,
author = {Kauermann, G. and Carroll, R. J.},
journal = {Journal of the American Statistical Association},
pages = {1387--1396},
title = {{A note on the efficiency of sandwich covariance matrix estimation}},
volume = {96},
year = {2001}
}
@article{Kerry2001,
author = {Kerry, Sally M. and Bland, J. M.},
journal = {Statistics in Medicine},
pages = {377--390},
title = {{Unequal cluster sizes for trials in English and Welsh general practice: Implications for sample size calculations}},
volume = {20},
year = {2001}
}
@article{Kristunas2017,
author = {Kristunas, Caroline A and Smith, Karen L and Gray, Laura J},
journal = {Trials},
pages = {109--119},
pmid = {28270224},
publisher = {Trials},
title = {{An imbalance in cluster sizes does not lead to notable loss of power in cross-sectional, stepped-wedge cluster randomised trials with a continuous outcome}},
volume = {18},
year = {2017}
}
@article{Kasza2017,
author = {Kasza, J. and Hemming, K. and Hooper, R. and Matthews, J. N.S. and Forbes, A. B.},
journal = {Statistical Methods in Medical Research},
title = {{Impact of non-uniform correlation structure on sample size and power in multiple-period cluster randomised trials}},
year = {2019},
volume = {28},
pages = {703--716},
}
@article{Kasza2018,
author = {Kasza, J. and Forbes, A. B.},
journal = {Statistical Methods in Medical Research},
title = {{Inference for the treatment effect in multiple-period cluster randomised trials when random effect correlation structure is misspecified}},
year = {2019},
volume = {28},
pages = {3112--3122},
}

% L
@article{Li2017,
author = {Li, Fan and Turner, Elizabeth L. and Heagerty, Patrick J. and Murray, David M. and Vollmer, William M. and Delong, Elizabeth R.},
issn = {10970258},
journal = {Statistics in Medicine},
title = {{An evaluation of constrained randomization for the design and analysis of group-randomized trials with binary outcomes}},
year = {2017},
volume={36},
pages={3791-3806}
}
@article{Liang1986,
author = {Liang, K.-Y. and Zeger, S. L.},
journal = {Biometrika},
pages = {13--22},
title = {{Longitudinal data analysis using generalized linear models}},
volume = {73},
year = {1986}
}
@article{Lu2007,
author = {Lu, B. and Preisser, J. S. and Qaqish, B. F. and Suchindran, C. and Bangdiwala, S. I. and Wolfson, M.},
journal = {Biometrics},
pages = {935--941},
title = {{A comparison of two bias-corrected covariance estimators for generalized estimating equations}},
volume = {63},
year = {2007}
}
@article{Li2018,
author = {Li, Fan and Turner, Elizabeth L. and Preisser, John S.},
journal = {Statistics and Probability Letters},
title = {{Optimal allocation of clusters in cohort stepped wedge designs}},
year = {2018},
volume={137},
pages={257--263}
}
@article{Li2015,
author = {Li, Fan and Lokhnygina, Yuliya and Murray, David M. and Heagerty, Patrick J. and Delong, Elizabeth R.},
issn = {10970258},
journal = {Statistics in Medicine},
pages = {1565--1579},
title = {{An evaluation of constrained randomization for the design and analysis of group-randomized trials}},
volume = {35},
year = {2015}
}
@article{Li2019,
author = {Li, F. and Forbes, A. B. and Turner, E. L. and Preisser, J. S.},
journal = {Statistics in Medicine},
pages = {636--649},
title = {{Power and sample size requirements for GEE analyses of cluster randomized crossover trials}},
volume = {38},
year = {2019}
}
@article{Li2017,
author = {Li, Fan and Turner, Elizabeth L. and Heagerty, Patrick J. and Murray, David M. and Vollmer, William M. and Delong, Elizabeth R.},
issn = {10970258},
journal = {Statistics in Medicine},
title = {{An evaluation of constrained randomization for the design and analysis of group-randomized trials with binary outcomes}},
year = {2017},
volume={36},
pages={3791-3806}
}
@article{LiReview2020,
author = {Li, F. and Hughes, J. P. and Hemming, K. and Taljaard, M. and Melnick, E. R. and Heagerty, P. J.},
journal = {Statistical Methods in Medical Research},
title = {{Mixed-effects models for the design and analysis of stepped wedge cluster randomized trials: An overview}},
year = {2020},
pages={10.1177/0962280220932962}
}
@article{LiTurnerPreisser2018,
author = {Li, F. and Turner, E. L. and Preisser, J. S.},
journal = {Biometrics},
pages = {1450--1458},
title = {{Sample size determination for GEE analyses of stepped wedge cluster randomized trials}},
volume = {74},
year = {2018}
}
@article{Li2020,
author = {Li, F.},
journal = {Statistics in Medicine},
title = {{Design and analysis considerations for cohort stepped wedge cluster randomized trials with a decay correlation structure}},
year = {2020},
volume = {4},
pages={438--495}
}
@article{Liu2002,
author = {Liu, A. and Shih, W. J. and Gehan, E.},
issn = {02776715},
journal = {Statistics in Medicine},
pages = {1787--1801},
title = {{Sample size and power determination for clustered repeated measurements}},
volume = {21},
year = {2002}
}

% M
@article{Manatunga2001,
author = {Manatunga, Amita K. and Hudgens, Michael G. and Chen, Shande},
doi = {10.1002/1521-4036(200102)43:1<75::AID-BIMJ75>3.0.CO;2-N},
journal = {Biometrical Journal},
pages = {75--86},
title = {{Sample size estimation in cluster randomized studies with varying cluster size}},
volume = {43},
year = {2001}
}
@article{Mancl2001,
author = {Mancl, L. A. and DeRouen, T. A.},
doi = {0.1111/j.0006-341X.2001.00126.x},
journal = {Biometrics},
pages = {126--134},
title = {{A covariance estimator for GEE with improved small-sample properties}},
volume = {57},
year = {2001}
}
@article{Martin2016b,
author = {Martin, J. and Girling, A. and Nirantharakumar, K. and Ryan, R. and Marshall, T. and Hemming, K.},
journal = {Trials},
pages = {402-413},
publisher = {Trials},
title = {{Intra-cluster and inter-period correlation coefficients for cross-sectional cluster randomised controlled trials for type-2 diabetes in UK primary care}},
volume = {17},
year = {2016}
}
@article{Murray1998b,
author = {Murray, David M. and Hannan, Peter J. and Wolfinger, Russell D. and Baker, William L. and Dwyer, James H},
journal = {Statistics in Medicine},
pages = {1581--1600},
title = {{Analysis of data from group-randomized trials with repeat observations on the same groups}},
volume = {17},
year = {1998}
}

@book{Murray1998,
author = {David M. Murray},
howpublished = {Hardcover},
publisher = {Oxford University Press},
address={New York, NY},
title = {{Design and Analysis of Group-Randomized Trials}},
year = {1998}
}
@article{maas2005sufficient,
  title={Sufficient sample sizes for multilevel modeling},
  author={Maas, Cora JM and Hox, Joop J},
  journal={Methodology},
  volume={1},
  pages={86--92},
  year={2005},
  publisher={Hogrefe \& Huber Publishers}
}

% P
@article{Pan2001,
  title={Sample size and power calculations with correlated binary data},
  author={Pan, Wei},
  journal={Controlled clinical trials},
  volume={22},
  pages={211--227},
  year={2001},
  publisher={Elsevier}
}
@article{Preisser2002,
author = {Preisser, John S. and Lohman, Kurt K. and Rathouz, Paul J.},
journal = {Statistics in Medicine},
pages = {3035--3054},
title = {{Performance of weighted estimating equations for longitudinal binary data with drop-outs missing at random}},
volume = {21},
year = {2002}
}
@article{Preisser2014,
author = {Preisser, John S. and Qaqish, Bahjat F.},
journal = {Journal of Statistical Computation and Simulation},
pages = {2441--2452},
title = {{A comparison of methods for simulating correlated binary variables with specified marginal means and correlations}},
volume = {84},
year = {2014}
}
@article{Preisser2008,
author = {Preisser, J. S. and Lu, B. and Qaqish, B. F.},
journal = {Statistics in Medicine},
mendeley-groups = {DCSWD},
pages = {5764--5785},
pmid = {19455509},
title = {{Finite sample adjustments in estimating equations and covariance estimators for intracluster correlations}},
volume = {27},
year = {2008}
}
@article{Perin2017,
author = {Perin, J. and Preisser, J. S.},
doi = {10.1111/biom.12614},
file = {:D$\backslash$:/A1 Methods Research/CRT Methodology/SWDBinomialGEE/References/Perin and Preisser 2017 Biometrics.pdf:pdf},
issn = {15410420},
journal = {Biometrics},
keywords = {Cluster randomized trials,Dental caries,Generalized Estimating Equations,Marginal association modeling,Small samples,Underage drinking},
pages = {696--705},
title = {{Alternating logistic regressions with improved finite sample properties}},
volume = {73},
year = {2017}
}
@article{Preisser1996,
author = {Preisser, John S. and Qaqish, Bahjat F.},
journal = {Biometrika},
pages = {551--562},
title = {{Deletion diagnostics for generalised estimating equations}},
volume = {83},
year = {1996}
}
@article{Preisser2003,
author = {Preisser, John S. and Young, Mary L. and Zaccaro, Daniel J. and Wolfson, Mark},
journal = {Statistics in Medicine},
pages = {1235--1254},
title = {{An integrated population-averaged approach to the design, analysis and sample size determination of cluster-unit trials}},
volume = {22},
year = {2003}
}
@article{Preisser2007,
author = {Preisser, John S and Reboussin, Beth A and Song, Eun Young and Wolfson, Mark},
isbn = {1044-3983},
issn = {1044-3983},
journal = {Epidemiology},
pages = {552--560},
title = {{The importance and role of intracluster correlations in planning cluster trials.}},
volume = {18},
year = {2007}
}
@article{Prost2015,
author = {Prost, Audrey and Binik, Ariella and Abubakar, Ibrahim and Roy, Anjana and {De Allegri}, Manuela and Mouchoux, Christelle and Dreischulte, Tobias and Ayles, Helen and Lewis, James J and Osrin, David},
journal = {Trials},
pages = {351-361},
publisher = {Trials},
title = {{Logistic, ethical, and political dimensions of stepped wedge trials: critical review and case studies.}},
volume = {16},
year = {2015}
}
@article{Prentice1988,
author = {Prentice, Ross L.},
journal = {Biometrics},
pages = {1033--1048},
pmid = {3233244},
title = {{Correlated binary regression with covariates specific to each binary observation.}},
volume = {44},
year = {1988}
}
@article{preisser2019population,
  title={A population-averaged approach to diagnostic test meta-analysis},
  author={Preisser, John S and Inan, Gul and Powers, James M and Chu, Haitao},
  journal={Biometrical Journal},
  volume={61},
  pages={126--137},
  year={2019},
  publisher={Wiley Online Library}
}

% Q
@article{Qaqish2003,
author = {Qaqish, B. F.},
journal = {Biometrika},
pages = {455--463},
title = {{A family of multivariate binary distributions for simulating correlated binary variables}},
volume = {90},
year = {2003}
}

% R
@article{Rochon1998,
author = {Rochon, James},
journal = {Statistics in Medicine},
pages = {1643--1658},
title = {{Application of GEE procedures for sample size calculations in repeated measures experiments}},
volume = {17},
year = {1998}
}
@article{Rubin1976,
author = {Rubin, DB},
journal = {Biometrika},
mendeley-groups = {SAMC},
pages = {581--592},
title = {{Inference and missing data}},
volume = {63},
year = {1976}
}
@article{ritz2004equivalence,
  title={Equivalence of conditional and marginal regression models for clustered and longitudinal data},
  author={Ritz, John and Spiegelman, Donna},
  journal={Statistical Methods in Medical Research},
  volume={13},
  pages={309--323},
  year={2004},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

% S
@article{Scott2014,
author = {Scott, JoAnna M and DeCamp, Allan and Juraska, Michal and Fay, Michael P and Gilbert, Peter B},
journal = {Statistical Methods in Medical Research},
title = {{Finite-sample corrected generalized estimating equation of population average treatment effects in stepped wedge cluster randomized trials}},
journal = {Statistical Methods in Medical Research},
volume = {26},
pages = {583-597},
year = {2017},
}
@article{Shih1997,
author = {Shih, W J},
journal = {Biometrical Journal},
pages = {899--908},
title = {{Sample size and power calculations for periodontal and other studies with clustered samples using the method of generalized estimating equations}},
volume = {39},
year = {1997}
}

% T
@article{Teerenstra2010,
author = {Teerenstra, Steven and Lu, Bing and Preisser, John S. and {Van Achterberg}, Theo and Borm, George F.},
journal = {Biometrics},
pages = {1230--1237},
title = {{Sample size considerations for GEE analyses of three-level cluster randomized trials}},
volume = {66},
year = {2010}
}
@article{Turner2017a,
author = {Turner, E. L. and Li, F. and Gallis, J. A. and Prague, M. and Murray, D. M.},
journal = {American Journal of Public Health},
pages = {907--915},
pmid = {28426295},
title = {{Review of recent methodological developments in group-randomized trials: part 1--design}},
volume = {107},
year = {2017},
}
@article{Turner2017b,
author = {Turner, E. L. and Prague, M. and Gallis, J. A. and Li, F. and Murray, D. M.},
journal = {American Journal of Public Health},
pages = {1078--1086},
pmid = {28426295},
title = {{Review of recent methodological developments in group-randomized trials: part 2--analysis}},
volume = {107},
year = {2017}
}
@article{Turner2019,
author = {Turner, Elizabeth L. and Yao, Lanqiu and Li, Fan and Prague, Melanie},
journal = {Statistical Methods in Medical Research},
title = {{Properties and pitfalls of weighting as an alternative to multilevel multiple imputation in cluster randomized trials with missing binary outcomes under covariate-dependent missingness}},
year = {2019}
}
@article{Thompson2018,
author = {Thompson, J. A. and Davey, C. and Fielding, K. and Hargreaves, J. R. and Hayes, R. J.},
journal = {Statistics in Medicine},
pages = {2487--2500},
title = {{Robust analysis of stepped wedge trials using cluster-level summaries within periods}},
volume = {37},
year = {2018}
}

@article{Taljaard2016,
author = {Taljaard, M. and Teerenstra, S. and Ivers, N. M. and Fergusson, D. A.},
journal = {Clinical Trials},
pages = {459--463},
title = {{Substantial risks associated with few clusters in cluster randomized and stepped wedge designs}},
volume = {13},
year = {2016}
}
@article{Thompson2017,
author = {Thompson, J. A. and Fielding, K. L. and Davey, C. and Aiken, A. M. and Hargreaves, J. R. and Hayes, R. J.},
issn = {10970258},
journal = {Statistics in Medicine},
pages = {3670--3682},
title = {{Bias and inference from misspecified mixed-effect models in stepped wedge trial analysis}},
volume = {36},
year = {2017}
}

% W
@article{Wedderburn1974,
author = {Wedderburn, R W M},
journal = {Biometrika},
pages = {439--447},
title = {{Quasi-likelihood functions, generalized linear models, and the Gauss-Newton method.}},
volume = {61},
year = {1974}
}
@article{white1982maximum,
  title={Maximum likelihood estimation of misspecified models},
  author={White, Halbert},
  journal={Econometrica: Journal of the Econometric Society},
  pages={1--25},
  year={1982},
  volume={50},
  publisher={JSTOR}
}

% Y
@article{yasui2004evaluation,
  title={Evaluation of community-intervention trials via generalized linear mixed models},
  author={Yasui, Yutaka and Feng, Ziding and Diehr, Paula and McLerran, Dale and Beresford, Shirley AA and McCulloch, Charles E},
  journal={Biometrics},
  volume={60},
  pages={1043--1052},
  year={2004},
  publisher={Wiley Online Library}
}
@article{Young2007,
author = {Young, Mary L. and Preisser, John S. and Qaqish, Bahjat F. and Wolfson, Mark},
journal = {Statistical Methods in Medical Research},
pages = {167--184},
title = {{Comparison of subject-specific and population averaged models for count data from cluster-unit intervention trials}},
volume = {16},
year = {2007}
}


% Z
@article{Zhou2020,
author = {Zhou, X. and Liao, X. and Kunz, L. M. and Normand, S-L. T. and Wang, M. and Spiegelman, D.},
journal = {Biostatistics},
volume = {1},
pages = {102--121},
title = {{A maximum likelihood approach to power calculations for stepped wedge designs of binary outcomes}},
year = {2020}
}
@article{Zeger1988,
author = {Zeger, S. L. and Liang, K.-Y. and Albert, P. S.},
journal = {Biometrics},
pages = {1049--1060},
title = {{Models for longitudinal data: A generalized estimating equation approach}},
volume = {44},
year = {1988}
}
@article{Zhao1990,
author = {Zhao, L. P. and Prentice, R. L.},
doi = {10.1093/biomet/77.3.642},
file = {:D$\backslash$:/A1 Methods Research/CRT Methodology/SWDSampSize/Reference/Zhao and Prentice Biometrika 2010.pdf:pdf},
issn = {00063444},
journal = {Biometrika},
keywords = {Binary regression,Correlated binary data,Estimating function,Multiplicative model,Pseudo-maximum likelihood,Quadratic exponential model},
pages = {642--648},
title = {{Correlated binary regression using a quadratic exponential model}},
volume = {77},
year = {1990}
}

@article{Henderson1981,
author = {Henderson, Harold V. and Searle, Shayle R.},
journal = {Siam Review},
pages = {53--60},
title = {{On deriving the inverse of a sum of matrices}},
volume = {23},
year = {1981}
}
@article{Sherman1950,
author = {Sherman, Jack and Morrison, Winifred J.},
journal = {Annals of Mathematical Statistics},
pages = {124--127},
title = {{Adjustment of an inverse matrix corresponding to a change in one element of a given matrix}},
volume = {21},
year = {1950}
}

@book{Graybill1983,
author = {Franklin A. Graybill},
howpublished = {Hardcover},
publisher = {Brooks/Cole},
address={Wadsworth, Belmont, CA},
title = {{Matrices with Applications in Statistics}},
year = {1983}
}

